Towards Co-execution on Commodity Heterogeneous Systems: Optimizations for Time-Constrained Scenarios

Heterogeneous systems are present from powerful supercomputers, to mobile devices, including desktop computers, thanks to their excellent performance and energy consumption. The ubiquity of these architectures in both desktop systems and medium-sized service servers allow enough variability to exploit a wide range of problems, such as multimedia workloads, video encoding, image filtering and inference in machine learning. Due to the heterogeneity, some efforts have been done to reduce the programming effort and preserve performance portability, but these systems include a set of challenges. The context in which applications offload the workload along with the management overheads introduced when doing co-execution, penalize the performance gains under time-constrained scenarios. Therefore, this paper proposes optimizations for the EngineCL runtime to reduce the penalization when co-executing in commodity systems, as well as algorithmic improvements when load balancing. An exhaustive experimental evaluation is performed, showing optimization improvements of 7.5\% and 17.4\% for binary and ROI-based offloading modes, respectively. Thanks to all the optimizations, the new load balancing algorithm is always the most efficient scheduling configuration, achieving an average efficiency of 0.84 under a pessimistic scenario.

==> rangetable.tex <==
\begin{tabular}{|c|c|c|c|}
   \hline
      Benchmark & Machine & $\frac{S_G}{S_C}$ within range & $\alpha_{opt}$ \\ \hline \hline
      Taylor & GTX950 & \begin{tikzpicture} \useasboundingbox (-0.4,-0.25) rectangle (2.5,0.2); \coordinate[label=below:0.718] (val) at (0,0); \coordinate[label=below:0.843] (min) at (1.1,0); \coordinate[label=below:8.531] (max) at (2.2,0); \draw (val) -- ($(min)!0.5!(max) $);
\draw[<->,double] (min) -- (max);
\node[circle,fill,inner sep=1pt] at (val) {};
\node[anchor=west] at (3,0) {};
\end{tikzpicture} & 0 \\ \hline
      Taylor & Kepler 758 & \begin{tikzpicture} \useasboundingbox (-0.4,-0.25) rectangle (2.5,0.2); \coordinate[label=below:0.888] (min) at (0,0); \coordinate[label=below:2.208] (val) at (1.1,0); \coordinate[label=below:3.400] (max) at (2.2,0); \draw (val) -- ($(min)!0.5!(max) $);
\draw[<->,double] (min) -- (max);
\node[circle,fill,inner sep=1pt] at (val) {};
\node[anchor=west] at (3,0) {};
\end{tikzpicture} & 0.31 \\ \hline
      Taylor & Kepler 324 & \begin{tikzpicture} \useasboundingbox (-0.4,-0.25) rectangle (2.5,0.2); \coordinate[label=below:0.253] (min) at (0,0); \coordinate[label=below:0.938] (val) at (1.1,0); \coordinate[label=below:1.920] (max) at (2.2,0); \draw (val) -- ($(min)!0.5!(max) $);
\draw[<->,double] (min) -- (max);
\node[circle,fill,inner sep=1pt] at (val) {};
\node[anchor=west] at (3,0) {};
\end{tikzpicture} & 0.52 \\ \hline
      Mandelbrot & GTX950 & \begin{tikzpicture} \useasboundingbox (-0.4,-0.25) rectangle (2.5,0.2); \coordinate[label=below:0.932] (val) at (0,0); \coordinate[label=below:0.943] (min) at (1.1,0); \coordinate[label=below:16.490] (max) at (2.2,0); \draw (val) -- ($(min)!0.5!(max) $);
\draw[<->,double] (min) -- (max);
\node[circle,fill,inner sep=1pt] at (val) {};
\node[anchor=west] at (3,0) {};
\end{tikzpicture} & 0 \\ \hline
      Mandelbrot & Kepler 758 & \begin{tikzpicture} \useasboundingbox (-0.4,-0.25) rectangle (2.5,0.2); \coordinate[label=below:0.842] (min) at (0,0); \coordinate[label=below:2.071] (val) at (1.1,0); \coordinate[label=below:2.593] (max) at (2.2,0); \draw (val) -- ($(min)!0.5!(max) $);
\draw[<->,double] (min) -- (max);
\node[circle,fill,inner sep=1pt] at (val) {};
\node[anchor=west] at (3,0) {};
\end{tikzpicture} & 0.33 \\ \hline
      Mandelbrot & Kepler 324 & \begin{tikzpicture} \useasboundingbox (-0.4,-0.25) rectangle (2.5,0.2); \coordinate[label=below:0.322] (min) at (0,0); \coordinate[label=below:0.892] (val) at (1.1,0); \coordinate[label=below:1.579] (max) at (2.2,0); \draw (val) -- ($(min)!0.5!(max) $);
\draw[<->,double] (min) -- (max);
\node[circle,fill,inner sep=1pt] at (val) {};
\node[anchor=west] at (3,0) {};
\end{tikzpicture} & 0.53 \\ \hline
      Nbody & GTX 950 & \begin{tikzpicture} \useasboundingbox (-0.4,-0.25) rectangle (2.5,0.2); \coordinate[label=below:1.407] (min) at (0,0); \coordinate[label=below:13.444] (max) at (1.1,0); \coordinate[label=below:17.746] (val) at (2.2,0); \draw (val) -- ($(min)!0.5!(max) $);
\draw[<->,double] (min) -- (max);
\node[circle,fill,inner sep=1pt] at (val) {};
\node[anchor=west] at (3,0) {};
\end{tikzpicture} & 1 \\ \hline
      Nbody & Kepler 758 & \begin{tikzpicture} \useasboundingbox (-0.4,-0.25) rectangle (2.5,0.2); \coordinate[label=below:0.906] (min) at (0,0); \coordinate[label=below:3.440] (max) at (1.1,0); \coordinate[label=below:7.901] (val) at (2.2,0); \draw (val) -- ($(min)!0.5!(max) $);
\draw[<->,double] (min) -- (max);
\node[circle,fill,inner sep=1pt] at (val) {};
\node[anchor=west] at (3,0) {};
\end{tikzpicture} & 1 \\ \hline
      Nbody & Kepler 324 & \begin{tikzpicture} \useasboundingbox (-0.4,-0.25) rectangle (2.5,0.2); \coordinate[label=below:0.236] (min) at (0,0); \coordinate[label=below:1.880] (max) at (1.1,0); \coordinate[label=below:3.137] (val) at (2.2,0); \draw (val) -- ($(min)!0.5!(max) $);
\draw[<->,double] (min) -- (max);
\node[circle,fill,inner sep=1pt] at (val) {};
\node[anchor=west] at (3,0) {};
\end{tikzpicture} & 1 \\ \hline
      Binomial & GTX950 & \begin{tikzpicture} \useasboundingbox (-0.4,-0.25) rectangle (2.5,0.2); \coordinate[label=below:0.755] (min) at (0,0); \coordinate[label=below:5.972] (max) at (1.1,0); \coordinate[label=below:9.789] (val) at (2.2,0); \draw (val) -- ($(min)!0.5!(max) $);
\draw[<->,double] (min) -- (max);
\node[circle,fill,inner sep=1pt] at (val) {};
\node[anchor=west] at (3,0) {};
\end{tikzpicture} & 1 \\ \hline
      Binomial & Kepler 758 & \begin{tikzpicture} \useasboundingbox (-0.4,-0.25) rectangle (2.5,0.2); \coordinate[label=below:0.722] (min) at (0,0); \coordinate[label=below:2.357] (max) at (1.1,0); \coordinate[label=below:7.922] (val) at (2.2,0); \draw (val) -- ($(min)!0.5!(max) $);
\draw[<->,double] (min) -- (max);
\node[circle,fill,inner sep=1pt] at (val) {};
\node[anchor=west] at (3,0) {};
\end{tikzpicture} & 1 \\ \hline
      Binomial & Kepler 324 & \begin{tikzpicture} \useasboundingbox (-0.4,-0.25) rectangle (2.5,0.2); \coordinate[label=below:0.201] (min) at (0,0); \coordinate[label=below:1.343] (max) at (1.1,0); \coordinate[label=below:3.356] (val) at (2.2,0); \draw (val) -- ($(min)!0.5!(max) $);
\draw[<->,double] (min) -- (max);
\node[circle,fill,inner sep=1pt] at (val) {};
\node[anchor=west] at (3,0) {};
\end{tikzpicture} & 1 \\ \hline
   \end{tabular}


==> sections/api.tex <==
\section{API Utilisation}
\label{sec:API}

%JLB: Cuidado con las etiquetas de los "listing"!!!!
Listings \ref{list:APIUtilisationBinomial} and \ref{list:APIUtilisationNBody} depict two benchmark examples using the EngineCL runtime, Binomial and NBody. Both programs start reading their kernels, defining variables, containers (\Cpp{} \textit{vectors}) and OpenCL values like \textit{local} and \textit{global work size} (\texttt{lws}, \texttt{gws}). Then, each program is initialised based on the benchmark (\texttt{init\_setup}), in lines 9 and 13 (\textit{L9,L13}), respectively. The rest of the program is where EngineCL is instantiated, used and released.



%JLB: Sería muy útil poner números de línea en el código y poder referirnos a ellas. Lo he visto en bastantes artículos.

%% \pagebreak

\begin{listing}[b] %% originally [!htb]
%\begin{snippet}[fontsize=\fontsize{6pt}{8.4pt}]{c++}
\begin{snippet}[fontsize=\footnotesize]{c++}
auto kernel = file_read("binomial.cl");
auto samples = 16777216; auto steps = 254;
auto steps1 = steps + 1; auto lws = steps1;
auto samplesBy4 = samples / 4;
auto gws = lws * samplesBy4;
vector<cl_float4> in(samplesBy4);
vector<cl_float4> out(samplesBy4);

binomial_init_setup(samplesBy4, in, out);

ecl::EngineCL engine;
engine.use(ecl::DeviceMask::CPU); // 1 Chip

engine.global_work_items(gws);
engine.local_work_items(lws);

ecl::Program program;
program.in(in);
program.out(out);

program.out_pattern(1, lws);

program.kernel(kernel, "binomial_opts");
program.arg(0, steps); // positional by index
program.arg(in); // aggregate
program.arg(out);
program.arg(steps1 * sizeof(cl_float4),
            ecl::Arg::LocalAlloc);
program.arg(4, steps * sizeof(cl_float4),
            ecl::Arg::LocalAlloc);

engine.use(std::move(program));

engine.run();

// if (engine.has_errors()) // [Optional lines]
//   for (auto& err : engine.get_errors())
//     show or process errors
\end{snippet}
%\vspace{-3mm}
\hyphenation{Binomial}
\caption{EngineCL API used in Binomial benchmark.}
\label{list:APIUtilisationBinomial}
\end{listing}

\begin{listing}[b] % originally !ht
%\begin{snippet}[fontsize=\fontsize{6pt}{8.4pt}]{c++}
\begin{snippet}[fontsize=\footnotesize]{c++}
auto kernel = file_read("nbody.cl");
auto gpu_kernel = file_read("nbody.gpu.cl");
auto igpu_kernel_bin =
  file_read_binary("nbody.igpu.cl.bin");
auto bodies = 512000; auto del_t = 0.005f;
auto esp_sqr = 500.0f; auto lws = 64;
auto gws = bodies;
vector<cl_float4> in_pos(bodies);
vector<cl_float4> in_vel(bodies);
vector<cl_float4> out_pos(bodies);
vector<cl_float4> out_vel(bodies);

nbody_init_setup(bodies, del_t, esp_sqr, in_pos,
                 in_vel, out_pos, out_vel);

ecl::EngineCL engine;
engine.use(ecl::Device(0, 0),
           ecl::Device(0, 1, igpu_kernel_bin),
           ecl::Device(1, 0, gpu_kernel));

engine.work_items(gws, lws);

auto props = { 0.08, 0.3 };
engine.scheduler(ecl::Scheduler::Static(props));

ecl::Program program;
program.in(in_pos);
program.in(in_vel);
program.out(out_pos);
program.out(out_vel);

program.kernel(kernel, "nbody");
program.args(in_pos, in_vel, bodies, del_t,
             esp_sqr, out_pos, out_vel);

engine.program(std::move(program));

engine.run();
\end{snippet}
%\vspace{-3mm}
\caption{EngineCL API used in NBody benchmark.}
\label{list:APIUtilisationNBody}
\end{listing}

Regarding the Binomial example, the \texttt{engine} \textit{uses} the first CPU in the system by using a \texttt{DeviceMask} (\textit{12}).
% , usually a single chip from the OpenCL Driver's point of view (\textit{L12}).
% Then, the \textit{global work size} (total number of work-items) and \textit{local work size} (work-items per work-group) are given to the engine using explicit methods (\textit{L14,15}).
% Then, the total number of work-items and work-items per work-group are given using explicit methods (\textit{L14,15}).
Then, the \textit{gws} and \textit{lws} are given by explicit methods (\textit{L14,15}).
% Now the application domain starts by instantiating the \texttt{program} (\textit{L17}). The input and output containers are set with \texttt{in} and \texttt{out} methods (\textit{L18,19}).
The application domain starts by creating the \texttt{program} and setting the input and output containers with methods \texttt{in} and \texttt{out} (\textit{L17-19}).
% With these statements the programmer notifies the runtime that the computation will need the values from the inputs before executing the kernel, but also that the outputs will be written after the execution.
%% This notifies the runtime that the computation will need the values from the inputs before executing the kernel and that the outputs will be written after the execution.
%% With these statements the runtime will manage the input and output buffers before and after the kernel execution.
With these statements the runtime manages and synchronises the input and output data before and after the computation. % the input values before the computation and the output values the input and output buffers before and after the kernel execution.
The \texttt{out\_pattern} is set because the implementation of the Binomial OpenCL kernel uses a writing pattern of $\frac{1\ out\ index}{255\ work-items}$ (\textit{L21}), that is, 255 work-items compute a single out index. Then, the kernel is configured by setting its source code string, name and arguments.
% The assignations are highly flexible, allowing to use transparently the previous containers (\textit{L23-29}).
Assignments are highly flexible, supporting aggregate and positional forms, and above all, it is possible to transparently use the variables and native containers (\textit{L23-29}).
% The above variables and containers can be used directly as kernel arguments. Also, the argument assignation can be done in aggregate and positional forms, allowing easy and flexible assignations (\textit{L24-29}).
% When local memory is needed, an enumerated \texttt{LocalAlloc} is used to determine that the assigned value represents the bytes of local memory to be reserved, reducing the complexity of the API.
The enumerated \texttt{LocalAlloc} is used to determine that the value represents the bytes of local memory that will be reserved, reducing the complexity of the API.
Finally, the runtime consumes the program and all the computation is performed (\textit{L32,34}). When the \texttt{run} method finishes, the output values are in the containers. % As shown in the comments, errors can be checked and processed easily.
 Optionally, errors can be checked and processed easily.
%%
%% // Optional:

%% On the other side, the NBody program shows a more advanced example where EngineCL really excels. In this example, three different kernels are shown: one is a common NBody kernel, other is a specific implementation for GPUs, and the third one is a binary kernel built for the Xeon Phi (\textit{L1-3}).
NBody program shows a more advanced example where EngineCL really excels. Three kernels are used: a common version, a specific implementation for GPUs and a binary kernel built for the integrated GPU (iGPU, \textit{L1-3}).
The \texttt{Device} class from the Tier-2 allows more features like
platform and device selection by index (\texttt{platform, device}) and specialisation of kernels and building options.
Three specific devices
% of the heterogeneous system
are instantiated, two of them with special kernels (source and binary) by just giving to them the file contents (\textit{L17}). After setting the work-items in a single method, the runtime is configured to use the \texttt{Static} scheduler with different work distributions for the CPU, integrated GPU and discrete GPU (\textit{L23,24}).
% If the proportions are not set, the scheduler will choose different distribution patterns like even or device-type distribution (e.g. GPU greater than CPU), depending on the runtime configuration (not shown in this example).
% Finally, the program is instantiated and defined.
Finally, the program is instantiated without any out pattern, because every work-item computes a single output value,
%($\frac{1}{1}$)
and the seven arguments are set in a single method, increasing the productivity even more (\textit{L33}).
%% Aquí estaba la otra figura listing2
As it is shown, EngineCL manages both programs with an easy and similar API, but completely changes the way it behaves: Binomial is executed completely in the CPU, while NBody is computed using the CPU, integrated GPU and discrete GPU with different kernel specialisations and workloads. Platform and device discovery, data management, compilation and specialisation, synchronisation and computation are performed transparently in a few lines for the programmer.

%% \vspace{-2mm}

==> sections/results_prev.tex <==
\section{Experimental Results}
\label{sec:Validation}

\subsection{Performance}
\label{sec:Performance}

%JLB: Quitar todo lo relativo a la SAPU. Añadir los nuevos experimentos.
This section presents results of experiments performed to evaluate the overhead introduced by EngineCL when a single kernel is executed in a single device and when using all the devices in the system with the Static and Dynamic schedulers.
%Figure \ref{fig:timeBatel} shows the overhead measured, comparing the OpenCL and EngineCL completion time for each problem size, in percentage. Each row presents the results of a different device, CPU, Xeon Phi and GPU, while each column corresponds to a benchmark.
%, Gaussian, Ray, Binomial, Mandelbrot and Nbody.
%% Five results are shown per benchmark, each one with a different problem size as it was explained in Section \ref{sec:Methodology}.
% It should be noted that negative overhead values indicate that running with EngineCL is more efficient (uses less time) than running natively with OpenCL.

The runtime overhead compared with OpenCL is on average around 0.46\% when using a single device. The worst results are obtained in the CPU, with an average (geometric mean) overhead of 0.68\%.
This is reasonable since EngineCL also runs on the CPU, so it interferes with the execution of benchmarks, stealing them computing capacity. Regarding the discrete devices, the Xeon Phi presents the best results with an average overhead of 0.18\%. Finally, the results achieved with the GPU are also excellent, with an average overhead of 0.26\%. The differences with GPU and Xeon Phi are explained by the different implementation of the OpenCL driver and how it is affected by the multi-threaded and optimised architecture of EngineCL.

% NOZ: Descartado para MULTIPROG2019
%\begin{figure}[!b]
%   \centering
%   %% \includegraphics[width=0.99\textwidth]{assets/charts_batel.pdf}
%   \includegraphics[width=0.49\textwidth]{assets/oclecl_overheads_40its_cpue5.pdf}
%   \includegraphics[width=0.49\textwidth]{assets/oclecl_overheads_40its_phi.pdf}
%   \includegraphics[width=0.49\textwidth]{assets/oclecl_overheads_40its_gputesla.pdf}
%   %% \vspace{-6mm}
%   \caption{Overheads in CPU Intel Xeon E5, Xeon Phi and NVIDIA GPU Tesla.}
%   \label{fig:timeBatel}
%\end{figure}

%% \begin{figure}[!hb]
%%    \centering
%%    %% \includegraphics[width=0.99\textwidth]{assets/charts_batel.pdf}
%%    \includegraphics[width=0.49\textwidth]{assets/charts_batel.pdf}
%%    %% \vspace{-2mm}
%%    \caption{Overheads in \textit{Batel} (CPU Intel Xeon E5, Xeon Phi and NVIDIA GPU Tesla).}
%%    \label{fig:timeBatel}
%% \end{figure}

%% \begin{figure}[!ht]
%%    \centering
%%    %% \includegraphics[width=0.99\textwidth]{assets/charts_apu.pdf}
%%    \includegraphics[width=0.49\textwidth]{assets/charts_apu.pdf}
%%    %% \vspace{-2mm}
%%    \caption{Overheads in \textit{APU} (AMD CPU A10-7850K with an integrated GPU R7).}
%%    \label{fig:timeAPU}
%% \end{figure}

%The GPU driver is less affected by the EngineCL management than the Phi driver.

% and its OpenCL management optimisations.
%JLB: La última frase de este párrafo, la he puesto por el comentario que me hiciste en el mail. Hay que explicarlo un poco más o simplemente quitarlo.
%JLB: Si puedes aportar alguna explicación más de los resultados es bienvenida.

%% \vspace{-10mm}
%% Figure \ref{fig:timeAPU} presents the same values as Figure \ref{fig:timeBatel} but evaluated in the \textit{APU} system. In this case the results for discrete devices are even better. For the CPU, the average overhead is only 0.12\% while the worst case is 0.98\%, practically negligible. With respect to the integrated GPU, most experiments show small gains, rather than losses, resulting in a negative mean overhead value of -0.12\%.

The performance results achieved in the heterogeneous system with different load balancing algorithms are shown in Figures \ref{fig:speedupBatel} and \ref{fig:efficiencyBatel}, where the speedups and efficiency are depicted, respectively. The abscissa axis shows the speedup and efficiency of the heterogeneous system for every scheduling configuration and benchmark. The ordinate axis contains the benchmarks defined in Section \ref{sec:Methodology}, each one with five scheduling configurations. The first two bars represent the Static algorithm varying the order of delivering the packages to the devices. The one labelled \emph{Static} delivers the first chunk to the CPU, the second to the Phi and the last one to the GPU, while in the \emph{Static rev} the order is \textit{gpu-phi-cpu}. The latter three show the Dynamic scheduler configured to run with 50, 100 and 150 chunks. These variations are presented to show the behaviours of the algorithms in different scenarios.
%The Static splits the total problem size in three chunks, one per device, with a chunk size based on the proportion of the computing power compared with the whole system.
%The order of the devices indicates how the problem is divided among them, that is, the first part of the problem for the first device (chunk 1), and so on.

The speedups presented in this section are due to the co-execution of the benchmarks on the CPU, Xeon Phi and GPU simultaneously, compared with only using the fastest device, the GPU. The efficiency gives an idea of how well a load is balanced. A value of 1.0 represents that all the devices have been working all the time, thus achieving the maximum obtainable speedup. The figures reveal that, for all benchmarks, there is at least one algorithm that offers excellent results with an efficiency of at least 0.84, except for Mandelbrot, where the efficiency is up to 0.76. Therefore, EngineCL can adapt to different kinds of loads obtaining outstanding performance.

Analysing the speedups and efficiencies in detail, Static delivers good results in regular applications, with consistent efficiencies between 0.80 and 0.87, regardless of the order of the devices. Binomial is an exception because the Xeon Phi's OpenCL Driver is penalised during the initialisation of the kernel (host-side) because it shares resources (threads) with the CPU, already computing. However, in irregular applications the results are much more erratic, because it does not adapt to these irregularities. For instance, there is a strong difference in efficiency between Ray1 (0.78) and Ray2 (0.92), being the same benchmark, but with different distribution of the input data. Furthermore, the order in which the devices are considered also has a significant impact on efficiency, as it is shown in Ray2 and Mandlebrot. The Mandelbrot set is irregular because it grows horizontally and the fractals are displaced to the bottom, having white areas in the top of the image. Therefore, when the slowest device (CPU) processes the first part of the image (chunk 1 in \textit{static}) it has better speedup than when it processes the last part (chunk 3 in \textit{static rev}), unbalancing the execution.

%The Static is the worst algorithm for irregular applications because it is not adaptive, such as Ray and Mandelbrot. Coming up with a balanced work distribution is significantly harder for Ray due to the complexity of interaction between the input scene and the ray tracing algorithm.  This is the same behavior with Ray, but instead of white areas, less objects and lights.

The Dynamic algorithm excels in most applications, achieving a geometric average efficiency of 0.81, but suffers in benchmarks like NBody and Gaussian. The former shows the overhead of communication when using many chunks and the latter the execution imbalance when using a few chunks,
% , reducing the communication overhead but increasing the work size and penalising a slow device.
increasing the work size and penalising the balancing due to slow devices.
Therefore, it is important to accurately determine the number of packages to get the best results in each benchmark.

%The analysis of the irregular benchmarks shows that the Dynamic method obtains the best results, with a geometric mean of 0.87 in efficiency. The Dynamic algorithm has good speedups in every irregular benchmark for any of the selected number of chunks, although the best selection depends on the benchmark (Ray1-Ray2 are 150, Ray3-Mandelbrot are 100).

\noindent\begin{minipage}{.49\textwidth}
\begin{figure}[H] % !t
   \centering
   %% \includegraphics[width=0.99\textwidth]{assets/charts_batel.pdf}
   \includegraphics[width=0.99\textwidth]{assets/benchmarks_speedup.pdf}
   \vspace{-2mm}
   \hyphenation{compared}
   \caption{Speedups for every scheduler compared with a single GPU.}
   \label{fig:speedupBatel}
\end{figure}
\end{minipage}
\hfill
\begin{minipage}{.49\textwidth}
\begin{figure}[H] % !t
   \centering
   %% \includegraphics[width=0.99\textwidth]{assets/charts_batel.pdf}
   \includegraphics[width=0.99\textwidth]{assets/benchmarks_efficiency.pdf}
   \vspace{-2mm}
   \caption{Efficiency of the system when adding the CPU and Xeon Phi.}
   \label{fig:efficiencyBatel}
\end{figure}
\end{minipage}
   \vspace{3mm}

%% Figure \ref{fig:worksizesBatel} depicts the work size distribution between the devices for every scheduler configuration and benchmark. Each bar has three rectangles with the work size given to each device. In the Static approach, the size is given by the proportions of computing power calculated offline, while in the Dynamic it is the final work size given at runtime.

%% Every scheduling configuration distributes a similar workload for each device, except in NBody and Mandelbrot.
%% The CPU takes more workload as the number of packages increases in NBody, introducing synchronisation overheads that are negligible when fewer packages are used. On the other side, Mandelbrot shows how the Phi processed too much amount of work for the part of the image given in the Static, being more complex to calculate than the expected when computing the complete image.

%% As it was introduced, the GPU in Binomial outperforms the CPU and Xeon Phi, as can be seen in the Static work size distributions. Therefore, a slightly variation in the completion time for any of these devices will imbalance the execution. Another important point is introduced to the analysis: the implementation of the OpenCL driver of the Xeon Phi needs and uses the CPU for its management. When using the CPU in co-execution, the Xeon Phi driver needs to share the CPU to build and manage the device with the CPU OpenCL driver, introducing time variations during the initialisation and new overheads in the final completion times. This behaviour is depicted in Figure \ref{fig:timingsBinomial}, showing the average times from initialisation for all the executions in Binomial, where the abscissa axis shows the base case (single device) and each scheduling configuration, with a bar showing the behaviour for each device. The ordinate axis shows the time since EngineCL started. Using only the Phi needs 1000 ms. to initialise and start computing, while it is up to 3000-4000 ms. when using in Static. This variation combined with the small amount of work given to the CPU and Phi produces enough imbalance to not achieve the goal. On the other side, the Dynamic approach it is much worth for two reasons: it allows small periods of CPU time without computation (between chunks) to the Phi driver and thanks to its adaptability solves the initialisation variations giving more chunks to the GPU, as it is shown.




%% new overheads during the initialisation and irregularities in the final  in the completion time due to the initialisation phase.
%% will Static approach suffers in Binomial not because of the  a penalty in Static approach

%% These benchmarks have not enough computation compared with the transference of data, therefore the communication overhead affects more, given sometimes even worse results than only using the Phi.

%Columns from left to right: gaussian, ray, binomial, mandelbrot, nbody.

%Rows from top to bottom: cpu-e5, phi, gpu-tesla.

%Min and Max overheads per device:
%\begin{itemize}
%\item cpu-e5 min -1.15\% max 2.69\%
%\item phi min -1.66\% max 0.98\%
%\item gpu-tesla min -0.12\% max 1.26\%
%\end{itemize}

%Average overheads and standard deviation per device:
%\begin{itemize}
%\item cpu-e5 1.08\% +- 1.11\%
%\item phi -0.29\% +- 0.74\%
%\item gpu-tesla 0.30\% +- 0.41\%
%\end{itemize}

%Columns from left to right: gaussian, ray, binomial, mandelbrot, nbody.

%Rows from top to bottom: cpu-a10, gpu-a10r7.

%Min and Max overheads per device:
%\begin{itemize}
%\item cpu-a10 min -1\% max 0.98\%
%\item gpu-a10r7 min -0.57\% max 0.35\%
%\end{itemize}

%Average overheads and standard deviation per device:
%\begin{itemize}
%\item cpu-a10 0.12\% +- 0.46\%
%\item gpu-a10r7 -0.12\% +- 0.25\%
%\end{itemize}




%% \noindent\begin{minipage}{.49\textwidth}
%% \begin{figure}[H] % !b
%%    \centering
%%    %% \includegraphics[width=0.99\textwidth]{assets/charts_batel.pdf}
%%    \includegraphics[width=0.99\textwidth]{assets/benchmarks_worksizes.pdf}
%%    %% \vspace{-2mm}
%%    \caption{Work size distribution per device and benchmark.}
%%    \label{fig:worksizesBatel}
%% \end{figure}
%% \end{minipage}
%% \hfill
%% \begin{minipage}{.49\textwidth}
%% \begin{figure}[H] % !b
%%    \centering
%%    %% \includegraphics[width=0.99\textwidth]{assets/charts_batel.pdf}
%%    \includegraphics[width=0.99\textwidth]{assets/timings_binomial.pdf}
%%    %% \vspace{-2mm}
%%    \caption{Binomial timings previous to the computation phase.}
%%    \label{fig:timingsBinomial}
%% \end{figure}
%% \end{minipage}

%\nota{Quizás prefieres que añada un resumencillo de la validación de rendimiento. La parte de análisis me ha parecido compleja de hacer, y en cosas como el binomial he ido más al detalle. No sé si habría que explicar algo más de Mandelbrot (su comportamiento en Dynamic), hacer más uso del speedup ya que tiendo a hablar de eficiencias porque son más uniformes). El mayor problema que estoy viendo es que ya alcanzamos 9 páginas.}

In summary, we can conclude that EngineCL can execute a single massive data-parallel kernel simultaneously on all devices in a heterogeneous system with negligible overhead. In addition, thanks to the load balancing algorithms, it yields excellent efficiencies, with different types of benchmarks.
